Multi-Agent Reinforcement Learning for Problems with Combined Individual and Team Reward

Many cooperative multi-agent problems require agents to learn individual tasks while contributing to the collective success of the group. This is a challenging task for current state-of-the-art multi-agent reinforcement algorithms that are designed to either maximize the global reward of the team or the individual local rewards. The problem is exacerbated when either of the rewards is sparse leading to unstable learning. To address this problem, we present Decomposed Multi-Agent Deep Deterministic Policy Gradient (DE-MADDPG): a novel cooperative multi-agent reinforcement learning framework that simultaneously learns to maximize the global and local rewards. We evaluate our solution on the challenging defensive escort team problem and show that our solution achieves a significantly better and more stable performance than the direct adaptation of the MADDPG algorithm.

==> ModelingBodyguard.tex <==
\section{The VIP Protection Problem}
\label{sec:ModelingBodyguard}

We are considering a VIP moving in a crowd of bystanders $\mathcal{B}=\left\{ b_{1},b_{2},\ldots,b_{m}\right\}$ protected from assault by a team of robot bodyguards $R=\left\{ r_{1},r_{2},\ldots,r_{n}\right\}$. To be able to reason about this problem, we need to quantify the {\em threat} to the VIP at a given moment - the aim of the bodyguards is to reduce this value.

We will use the threat model defined in~\cite{Bhatia-2016-FLAIRS}. Two agents $x$ and $y$ have a {\em line of sight} $LoS(x,y)\in\left[0,1\right]$ if $x$ can directly observe $y$ and with no obstacle between them. A bystander $b$ can only pose a threat to the VIP if it is closer than the safe distance $\mathrm{SafeDist}$. The {\em threat level} $\mathrm{TL}\left(\mathrm{VIP},b\right)$ is defined as the probability
that a bystander $b$ can successfully assault the VIP, defined as a value exponentially decaying with distance:
\begin{equation}
\mathrm{TL}\left(\mathrm{VIP},b\right)=\exp^{-A\left(\mathrm{Dist}(\mathrm{VIP},b)\right)/B}
\end{equation}
\noindent where the VIP should be in line of sight of $b$ and  $\mathrm{Dist}(\mathrm{VIP},b)<\mathrm{SafeDist}$. $A$ and $B$ are positive constants that control the decay rate of the threat level.

%The cumulative threat to the VIP from crowd $\mathcal{B}$ in the absence of bodyguards over the time $T$ is defined as:
%\begin{equation}
%\label{eq:ct}
%\mathrm{CT}=\intop_{0}^{T}1-\prod_{i=1}^{k}\left(1-\mathrm{TL}\left(\mathrm{VIP},b\right)\right)dt
%\end{equation}
%The cumulative threat to the VIP depends on the movement of the VIP and the distance of the bystanders.

The residual threat $RT\left(VIP, \mathcal{B}, R\right)$ is defined as the threat to the VIP at time $t$ from bystanders $\mathcal{B}$. Bodyguards can block the line of sight from the bystanders, thus the residual threat is always smaller than the threat level and depends on the position of the bodyguards with respect to the bystanders and the VIP. The {\em cumulative residual threat} to the VIP from bystanders $\mathcal{B}$ in the presence of bodyguards $R$ over the time period $[0,T]$ is defined as:
\begin{equation}
\label{eq:crt}
\mathrm{CRT}=\intop_{0}^{T}1-\prod_{i=1}^{k}\left(1-RT\left(VIP,b_{i}, R\right)\right)dt
\end{equation}
Our end goal is to minimize $\mathrm{CRT}$ through multi-agent reinforcement learning.

